Degradation Aware Predictive Energy Management Strategy for Ship Power Systems

Integration of modern defence weapons into ship power systems poses a challenge in terms of meeting the high ramp rate requirements of those loads. It might be demanding for the generators to meet the ramp rates of these loads. Failure to meet so, might lead to stability issues. This is addressed by conglomeration of generators and energy storage elements to handle the required power demand posed by loads. This paper proposes an energy management strategy based on model predictive control that incorporates the uncertainty in the load prediction. The proposed controller optimally coordinates the power split between the generators and energy storage elements to guarantee that the power demand is met taking into considerations the ramp rate limitations and the load uncertainty. A low bandwidth model consisting of a single generator and a single energy storage element is used to validate the results of the proposed energy management strategy. The results demonstrate the robustness of the controller under load prediction uncertainty and demonstrate the effect of load uncertainty on battery capacity loss.

==> FinalVersion/control_development.tex <==
% \section{Control Development}
This section presents the development and derivation of the proposed EM strategy. Consider the MPC problem of the form:
\begin{equation}\label{MPC_main}
\begin{aligned}
\Minimize \quad & \sum_{\text{k}=1}^{\text{h}}  \frac{\beta}{2}\norm{\mathbf{l}_\text{k}-\textbf{l}_\text{k}^\text{f}}_\text{W}^2+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\text{x}_{\text{k}_\text{j}})\\
\textrm{s.t.} \quad &  \underline{\textbf{1}}^\text{T}\textbf{x}_\text{k} = \underline{\textbf{1}}^\text{T}\textbf{l}_\text{k}, \hspace{2mm} \textbf{x}_\text{k} \in \mathbb{R}^{\text{n}_\text{x}}, \textbf{l}_\text{k} \in \mathbb{R}^{\text{n}_\text{l}} \\
& \textbf{x}_\text{j} \in \mathbb{\chi}_\text{j},\hspace{3mm} \text{j} = 1,...,\text{n}_\text{x}  \\
\end{aligned}
\end{equation}

Where $\text{h} \in \mathbb{N}$ represents the prediction horizon, $\text{n}_\text{x} \in \mathbb{N}$ represents the number of distributed energy resources (DERs) such as generators and ESSs, $\text{n}_\text{l} \in \mathbb{N}$ denotes the number of loads, in our case PMMs. $\textbf{l}_\text{k}^\text{f} \in \mathbb{R}^{\text{n}_\text{l}}$ is the forecasted load vector at future time $\text{k}$. $\textbf{l}_\text{k} \in \mathbb{R}^{\text{n}_\text{l}}$ is the decision vector capturing the total power supplied to each load bus at future time $\text{k}$. $\textbf{x}_\text{k} \in \mathbb{R}^{\text{n}_\text{k}}$ is the decision vector capturing the total power injected by the DERs at future time $\text{k}$. $\text{C}_\text{j}:\mathbb{R}\longrightarrow\mathbb{R}_+$ is the cost associated with the power injected by the $\text{j}^{th}$ DER. The cost function for the generator could capture the efficiency map and for the ESSs it could capture the effective life degradation. $\mathcal{\chi}_\text{j} \subset \mathbb{R}^\text{h}$ represents the convex set for each DER summarizing attributes such as upper and lower power limits, ramp rate limits and relevant system dynamics. $\text{W} \in \mathbb{R}^{\text{n}_\text{l} \times \text{n}_\text{l}}$ is a positive definite weight matrix penalizing the power mismatch between forecasted load and supplied power.

\begin{proposition}
The optimization problem in (\ref{MPC_main}) is equivalent to the following problem: 
\begin{equation}\label{MPC_two}
\begin{aligned}
\Minimize \quad & \sum_{\text{k}=1}^{\text{h}}  \frac{\alpha}{2}(\underline{\textbf{1}}^\text{T}\textbf{x}_\text{k}-\text{m}_\text{k}^\text{f})+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\text{x}_{\text{k}_\text{j}})\\
\textrm{s.t.} \quad & \textbf{x}_\text{j} \in \mathbb{\chi}_\text{j}\\
\end{aligned}
\end{equation}
Where $$\text{m}_\text{k} = \underline{\textbf{1}}^\text{T}\textbf{l}_\text{k}^\text{f}$$ $$\alpha = \frac{\beta}{\underline{\textbf{1}}^\text{T}\text{W}\underline{\textbf{1}}}$$
\end{proposition}
\textit{Proof:} The Lagrangian for the problem (\ref{MPC_main}) is
\begin{equation}
    \mathcal{L} = \sum_{\text{k}=1}^{\text{h}} \bigg(\frac{\beta}{2}\norm {\textbf{l}_\text{k}-\textbf{l}_\text{k}^\text{f}}_\text{W}^2+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\text{x}_{\text{k}_\text{j}})+\lambda_\text{k}(\underline{\textbf{1}}^\text{T}\textbf{x}_\text{k}-\underline{\textbf{1}}^\text{T}\textbf{l}_\text{k})\bigg)+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{I}_{\mathcal{\chi}_\text{j}}
\end{equation}
Where $\lambda_\text{k} \in \mathbb{R}$ is the associated Lagrange multiplier for the equality constraint and $\text{I}_{\mathcal{\chi}_\text{j}}$ is an indicator function of the convex set $\mathcal{\chi}_\text{j}$. Taking derivative with respect to $\textbf{l}_\text{k}$ and $\lambda_\text{k}$ and equaling to zero yields the first order optimality conditions we get: $$\beta \text{W}(\textbf{l}_\text{k}-\textbf{l}_\text{k}^\text{f})-\lambda_\text{k} \underline{\textbf{1}} = 0$$ $$\underline{\textbf{1}}^\text{T}\textbf{x}_\text{k} = \underline{\textbf{1}}^\text{T}\text{l}_\text{k}$$
Which implies that $$\lambda_\text{k} = \frac{\beta}{\underline{\textbf{1}}^\text{T}\text{W}^{-1}\underline{\textbf{1}}}(\underline{\textbf{1}}^\text{T}\textbf{x}_\text{k}-\underline{\textbf{1}}^\text{T}\textbf{l}_\text{k}^\text{f})$$ and 
$$\norm{\textbf{l}_\text{k}-\textbf{l}_\text{k}^\text{f}}_\text{W}^2 = \frac{1}{\underline{\textbf{1}}^\text{T}\text{W}^{-1}\underline{\textbf{1}}}(\underline{\textbf{1}}^\textbf{T}\textbf{x}_\text{k}-\textbf{m}_\text{k})^2$$
Therefore
\begin{equation}
    \mathcal{L} = \sum_{\text{k}=1}^{\text{h}}  \bigg(\frac{\alpha}{2}(\underline{\textbf{1}}^\text{T}\textbf{x}_\text{k}-\text{m}_\text{k})^2+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\text{x}_{\text{k}_\text{j}})\bigg)+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{I}_{\mathcal{\chi}_\text{j}}
\end{equation}
which is the corresponding Lagrangian for problem (\ref{MPC_two}).
\begin{remark}
The optimization problem in (\ref{MPC_two}) could have been written directly from the problem statement. However, what is not obvious is how the relative weight matrix $\text{W}$ is aggregated into a scalar weight for the total demand-supply tracking error in (\ref{MPC_two})
\end{remark}

\subsection{Algorithm via ADMM}
In this section, the ADMM technique is used to split the problem (\ref{MPC_two}) into $\text{n}_\text{x}$ local optimization problems which are coupled via an aggregator or scheduler which is implementing the Lagrange multiplier update between each iteration. First, the problem in (\ref{MPC_two}) is written as:
\begin{equation}\label{MPC_ADMM}
\begin{aligned}
\Minimize \quad & \frac{\alpha}{2} \sum_{\text{k}=1}^{\text{h}} \bigg(\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{y}_{\text{j}_\text{k}}-\text{m}_\text{k}\bigg)^2+\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\text{x}_\text{j})\\
\textrm{s.t.} \quad & \text{x}_\text{j} = \text{y}_\text{j} \\
  & \textbf{x}_\text{j} \in \mathcal{\chi}_\text{j}   \\
\end{aligned}
\end{equation}
Where $\text{y}_\text{j} \in \mathbb{R}^\text{h}$ is dummy variable which is introduced to split the problem and  $\text{C}_\text{j}(\text{x}_\text{j}) \triangleq \sum_{\text{k}=1}^{\text{h}}\text{C}_\text{j}{\text{x}_{\text{k}_\text{j}}} $ is the total cost for each DER.

Let $\lambda_\text{j} \in \mathbb{R}^\text{h}$ be the Lagrange multiplier associated with the equality constraint $\text{x}_\text{i}$ = $\text{y}_\text{j}$. The augmented Lagrangian for the problem (\ref{MPC_ADMM}) is given as:
\begin{equation}
\begin{split}
  \mathcal{L}_{\rho} = \frac{\alpha}{2}\sum_{\text{k}=1}^{\text{h}}\big(\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{y}_{\text{j}_\text{k}}-\text{m}_\text{k}\big)^2+\sum_{\text{j}=1}^{\text{n}_\text{x}}\bigg(\text{C}_\text{j}(\text{x}_\text{j})+\\\frac{\rho}{2}\norm{\text{x}_\text{j}-\text{y}_\text{j}+\text{u}_\text{j}}^2-\frac{\rho}{2}\norm{\text{u}_\text{j}}^2+\text{I}_{{\mathcal{\chi}}_\text{j}}\bigg)
\end{split}
\end{equation}
Where $\text{u}_\text{j} = \frac{1}{\rho}\lambda_\text{j}$ is a scaled Lagrange multiplier with $\rho \in \mathbb{R}_+$.
The following successive optimization problems are considered:
\begin{subequations}\label{ADMM Scaled Optimization}
\begin{align}
    \text{y}_\text{j}^{\text{t}+1} &= \argmin \frac{\alpha}{2}\sum_{\text{k}=1}^{\text{h}}\big(\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{y}_{\text{j}_\text{k}}-\text{m}_\text{k}\big)^2+\frac{\rho}{2}\sum_{\text{j}=1}^{\text{n}_\text{x}}\norm{\text{x}_\text{j}^\text{t}-\text{y}_\text{j}+\text{u}_\text{j}^\text{t}}^2 \\
    \text{x}_\text{j}^{\text{t}+1} &= \argmin_{\text{x}_\text{j} \in \mathcal{\chi}_\text{j}} \text{C}_\text{j}(\text{x}_\text{j})+\frac{\rho}{2}\norm{\text{x}_\text{j}-\text{y}_\text{j}^{\text{t}+1}+\text{u}_\text{j}}^2 \\
    \text{u}_\text{j}^{\text{t}+1} &= \text{u}_\text{j}+\text{x}_\text{j}^{\text{t}+1}-\text{y}_\text{j}^{\text{t}+1}
\end{align}
\end{subequations}
While (\ref{ADMM Scaled Optimization}a) and (\ref{ADMM Scaled Optimization}b) can be executed in parallel, it is not straightforward for (\ref{ADMM Scaled Optimization}a). However, the optimization problem in (\ref{ADMM Scaled Optimization}a) is unconstrained quadratic program that can be solved analytically. We derive the solution and identify the underlying aggregator scheme. The first order optimality conditions for (\ref{ADMM Scaled Optimization}a) are as follows:
$$\alpha \sum_{\text{k}=1}^{\text{h}}\big(\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{y}_{\text{j}_\text{k}}-\text{m}_\text{k}\big)-\rho(\text{x}_\text{j}^\text{t}-\text{y}_\text{j}+\text{u}_\text{j}^\text{t}) = 0$$
Expanding the above equation through entire horizon and after some mathematical manipulations we arrive at:
\begin{equation}
    \text{y}_\text{j} = \text{x}_\text{j}^\text{t}+\text{u}_\text{j}^\text{t}+\frac{\alpha}{\alpha \text{n}_\text{x}+\rho}\bigg(\text{m}-\sum_{\text{j}=1}^{\text{n}_\text{x}}(\text{x}_\text{j}^\text{t}+\text{u}_\text{j}^\text{t})\bigg)
\end{equation}
Thus each node implements the following at each iteration $\text{t}$
\begin{subequations}
\begin{align}
    \text{x}_\text{j}^{\text{t}+1} &= \argmin_{\text{x}_\text{j} \in \mathcal{\chi}_\text{j}} \text{C}_\text{j}(\text{x}_\text{j})+\frac{\rho}{2}\norm{\text{x}_\text{j}-\text{x}_\text{j}^\text{t}-\text{a}^\text{t}}_2^2 \\
    \text{z}_\text{j}^{\text{t}+1} &= 2\text{x}_\text{j}^{\text{t}+1}-\text{x}_\text{j}^\text{t}-\text{a}^\text{t}
\end{align}
\end{subequations}
Where $$\text{a}^\text{t} = \frac{\alpha}{\alpha \text{n}_\text{x}+\rho}\bigg(\text{m}-\sum_{\text{j}=1}^{\text{n}_\text{x}}\underbrace{(\text{x}_\text{j}^\text{t}+\text{u}_\text{j}^\text{t})}_{\text{z}_{\text{j}}^\text{t}}\bigg)$$ is the aggregator output sent to all nodes.


\subsection{Generator Node Optimization Problem}
In this subsection we will be using the following generator specific notation $\textbf{x}_\text{j} \triangleq \textbf{p}_{\text{g}_\text{j}}$. The assumption is that, all the generators implement constant power sharing via droop control i.e $\textbf{p}_{\text{g}_\text{j}} = \theta_\text{i}\textbf{p}_\text{g}$ with $\sum_{\text{j}=1}^{\text{n}_\text{x}}\theta_\text{j}=1$ where $\textbf{p}_\text{g} \in \mathbb{R}^\text{h}$ is the total generation profile for the horizon. The generation cost $\text{C}_\text{g}(\text{p}_\text{g}) \triangleq \sum_{\text{k}=1}^{\text{h}}\sum_{\text{j}=1}^{\text{n}_\text{x}}\text{C}_\text{j}(\theta_\text{j}\text{p}_{\text{g}_\text{k}})$. In this paper, the cost function is considered to be smooth and quadratic. The resulting optimization problem at the generator node is given as:
\begin{equation}
\begin{aligned}
\Minimize \quad & \text{C}_\text{g}(\text{p}_\text{g})+\frac{\rho}{2}\norm{\textbf{p}_\text{g}-\textbf{p}_\text{g}^\text{t}-\textbf{a}^\text{t}}^2\\
\textrm{s.t.} \quad & 0 \preceq \textbf{p}_\text{g} \preceq \frac{\overline{\textbf{p}}_\text{g}}{\overline{\theta}}\underline{\textbf{1}}\\
& \begin{bmatrix} D \\ -D \end{bmatrix}\textbf{p}_\text{g} \preceq \frac{\text{r}_\text{g}\overline{\textbf{p}}_\text{g}}{\overline{\theta}}\underline{\textbf{1}}
\end{aligned}    
\end{equation}
Where $\overline{\theta} \triangleq \max_{\text{j}}\{\theta_\text{j}\}$. $\text{r}_\text{g}$ is the ramp rate limitation of the generator. $\overline{\textbf{p}}_\text{g}$ represents the upper power limitations on generator power and $D$ represents the rate matrix associated with ramp rate limitation of generator throughout the horizon. The output sent to the aggregator is as follows:
\begin{equation}
    \text{z}_\text{g}^{\text{t}+1} = 2\text{p}_\text{g}^*-\text{p}_\text{g}^\text{t}-\text{a}^{\text{t}}
\end{equation}

\subsection{ESS Node Optimization problem}
The assumption that battery can operate bidirectionally is made. The optimization problem at the ESS node is given as:
\begin{equation}
\begin{aligned}
\Minimize \quad & \frac{\rho}{2}\norm{\textbf{p}_\text{b}-\textbf{p}_\text{b}^\text{t}-\textbf{a}^\text{t}}^2\\
\textrm{s.t.} \quad & \underline{\textbf{1}}^\text{T}\textbf{p}_\text{b} = \frac{3600\text{Q}_\text{T}\text{v}_\text{b}^*}{\text{T}_\text{s}}(\text{q}_0-\text{q}_\text{h})\\ & \begin{bmatrix} D \\ -D \end{bmatrix}\textbf{p}_\text{b} \preceq \text{r}_\text{b}\underline{\textbf{1}}\\
& \underline{\textbf{p}}_\text{b} \preceq \textbf{p}_\text{b} \preceq \overline{\textbf{p}}_\text{b}
\end{aligned}    
\end{equation}
Where $\text{Q}_\text{T}$ represents the total capacity of the battery. $\text{v}_\text{b}^*$ denotes the bus voltage. $\text{q}_0$ and $\text{q}_\text{h}$ represent initial SoC and SoC at the end of horizon. $\text{T}_\text{s}$ is the Euler discretization sampling time. $\text{r}_\text{b}$ represents the ramp rate of the ESSs. $\underline{\textbf{p}}_\text{b}$ and $\overline{\textbf{p}}_\text{b}$ are the lower and the upper power limitations on the ESS respectively. The output from ESSs nodes sent to the aggregator is as follows:
\begin{equation}
    \text{z}_\text{b}^{\text{t}+1} = 2\text{p}_\text{b}^*-\text{p}_\text{b}^\text{t}-\text{a}^{\text{t}}
\end{equation}

\begin{figure}[h!] 
	\centering
	\includegraphics[width=0.33\textwidth]{Figures/ADMM_SPS.png} 
	\caption{Controller Structure for SPS. 
    }
	\label{SPS_ADMM}
\end{figure}


  


